A Practical Approach to Polar Codes

In this paper, we study polar codes from a practical point of view. In particular, we study concatenated polar codes and rate-compatible polar codes. First, we propose a concatenation scheme including polar codes and Low-Density Parity-Check (LDPC) codes. We will show that our proposed scheme outperforms conventional concatenation schemes formed by LDPC and Reed-Solomon (RS) codes. We then study two rate-compatible coding schemes using polar codes. We will see that polar codes can be designed as universally capacity achieving rate-compatible codes over a set of physically degraded channels. We also study the effect of puncturing on polar codes to design rate-compatible codes.

==> IEEEtran/README <==

December 10, 2002

This IEEEtran.cls is now the official LaTeX class for authors of the
Institute of Electrical and Electronics Engineers (IEEE) transactions
journals and conferences. IEEEtran.cls is mirrored within IEEE's site
as well.

The most recent version of IEEEtran.cls is version 1.6b. IEEEtran.cls now
provides support for conferences and A4 paper. Users of previous versions
should no longer manually alter margins, paper sizes, page styles, etc.
Also, please note that \author is used slightly differently from that of
V1.5, especially for conferences. \pubid (if used) must now be placed
before \maketitle. \cite is now robust and can be used within captions
without a proceeding \protect.

As with previous versions, The itemize, enumerate, and description lists as
well as \appendix(ces) have enhanced controls and work slightly differently
than is done in traditional LaTeX.

Extensive formal documentation is now available. Enjoy! ;) The appendices
of the user manual contain important information on avoiding commonly
made mistakes, compatibility issues and installation instructions.


Best wishes for all your publication endeavors,

Michael Shell
mshell@ece.gatech.edu


*******
Version 1.6b (2002/11/18) changes:

 1) New peerreview and peerreviewca modes with \IEEEpeerreviewmaketitle
    command allows for a "cover" titlepage for anonymous peer review.

 2) New draftclsnofoot mode is like draftcls, but does not display the
    date and the word "DRAFT" at the foot of the page. 

 3) The draft modes now no longer force a pagebreak after the title.

 4) \table* now defaults to \footnotesize text like \table.

 5) In addition to the IEEE IED lists, the original IED style list
    environments (as is done in article.cls) are now provided as
    LaTeXitemize, LaTeXenumerate, and LaTeXdescription. Also, users
    can now redefine \makelabel within IEEE IED list controls.

 6) Added \special to feed papersize to dvips.

 7) Revised font selection method so as not to have problems when used
    with setspace.sty. 

 8) Extra code to prevent hyperref.sty from interfering with the operation
    of cite.sty.

 9) Fixed problem with figure captions when using hyperref.sty.



***************** Subdirectories *****************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************* Files **********************

README             - This file.

IEEEtran.cls       - The LaTeX class file.

IEEEtran_HOWTO.pdf - The user manual.

bare_conf.tex      - A "bare bones" starter file for conference papers.

bare_jrnl.tex      - A "bare bones" starter file for journal papers.




**********************************************************************
 Legal Notice:
 This code and advice is offered as-is without any warranty either
 expressed or implied; without even the implied warranty of
 MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE!
 User assumes all risk.
 In no event shall IEEE or any contributor to this code
 be liable for any damages or losses, including, but not limited to,
 incidental, consequential, or any other damages, resulting from the
 use or misuse of any information contained here.
 
 All statements made here are the opinions of their respective
 authors and are not necessarily endorsed by the IEEE.

 This code/text is distributed under the Perl Artistic License 
 ( http://language.perl.com/misc/Artistic.html ) 
 and may be freely used, distributed and modified.
 Retain all contribution notices and credits.
**********************************************************************




==> IEEEtran/tools/README <==

December 10, 2002

The IEEEtrantools.sty package provides several commands from the IEEEtran.cls
file so that they can be used under other LaTeX classes. The user guide
provided here covers only the differences in the use of the commands from
those provided by IEEEtran.cls. For complete documentation on these commands,
see the relevant sections in the IEEEtran_HOWTO manual of the IEEEtran LaTeX
class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \PARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.


Michael Shell
mshell@ece.gatech.edu


*******
Version 1.1 (2002/11/18) changes:

 1) In addition to the IEEE IED lists, the original LaTeX IED style lists
    environments are now preserved as LaTeXitemize, LaTeXenumerate, and
    LaTeXdescription. Also, users can now redefine \makelabel within
    IEEE IED list controls.


********************* Files **********************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.




**********************************************************************
 Legal Notice:
 This code and advice is offered as-is without any warranty either
 expressed or implied; without even the implied warranty of
 MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE!
 User assumes all risk.
 In no event shall IEEE or any contributor to this code
 be liable for any damages or losses, including, but not limited to,
 incidental, consequential, or any other damages, resulting from the
 use or misuse of any information contained here.
 
 All statements made here are the opinions of their respective
 authors and are not necessarily endorsed by the IEEE.

 This code/text is distributed under the Perl Artistic License 
 ( http://language.perl.com/misc/Artistic.html ) 
 and may be freely used, distributed and modified.
 Retain all contribution notices and credits.
**********************************************************************



